Garbage Collection for Rust: The Finalizer Frontier

Rust is a non-Garbage Collected (GCed) language, but the lack of GC makes expressing data-structures that require shared ownership awkward, inefficient, or both. In this paper we explore a new design for, and implementation of, GC in Rust, called Alloy. Unlike previous approaches to GC in Rust, Alloy allows existing Rust destructors to be automatically used as GC finalizers: this makes Alloy integrate better with existing Rust code than previous solutions but introduces surprising soundness and performance problems. Alloy provides novel solutions for the core problems: finalizer safety analysis rejects unsound destructors from automatically being reused as finalizers; finalizer elision optimises away unnecessary finalizers; and premature finalizer prevention ensures that finalizers are only run when it is provably safe to do so.

==> tables/gcvs_perf_individual.tex <==
\begin{tabular}{l l @{\hspace{6pt}}r@{\hspace{3pt}}l @{\hspace{6pt}}r@{\hspace{3pt}}l @{\hspace{6pt}}r@{\hspace{3pt}}l @{\hspace{6pt}}r@{\hspace{3pt}}l @{\hspace{6pt}}r@{\hspace{3pt}}l @{\hspace{6pt}}r@{\hspace{3pt}}l}
\toprule
Suite & Benchmark & \multicolumn{6}{c}{Wallclock-time (seconds)} & \multicolumn{6}{c}{User-time (seconds)} \\
 &  & \multicolumn{2}{c}{RC \texttt{[jemalloc]}} & \multicolumn{2}{c}{Alloy \texttt{[default]}} & \multicolumn{2}{c}{RC \texttt{[gcmalloc]}} & \multicolumn{2}{c}{RC \texttt{[jemalloc]}} & \multicolumn{2}{c}{Alloy \texttt{[default]}} & \multicolumn{2}{c}{RC \texttt{[gcmalloc]}} \\
\midrule
\multirow{10}{*}{\rotatebox{90}{alacritty}} & Cur. Motion & 0.65 & \scriptsize\textcolor{gray!60}{[0.63,0.66]} & 0.66 & \scriptsize\textcolor{gray!60}{[0.65,0.66]} & 0.66 & \scriptsize\textcolor{gray!60}{[0.65,0.67]} & 1.08 & \scriptsize\textcolor{gray!60}{[1.03,1.14]} & 1.09 & \scriptsize\textcolor{gray!60}{[1.04,1.13]} & 1.09 & \scriptsize\textcolor{gray!60}{[1.05,1.13]} \\
 & Dense Cells & 2.16 & \scriptsize\textcolor{gray!60}{[2.14,2.19]} & 2.16 & \scriptsize\textcolor{gray!60}{[2.14,2.18]} & 2.14 & \scriptsize\textcolor{gray!60}{[2.10,2.18]} & 6.66 & \scriptsize\textcolor{gray!60}{[6.53,6.79]} & 6.62 & \scriptsize\textcolor{gray!60}{[6.51,6.74]} & 6.58 & \scriptsize\textcolor{gray!60}{[6.43,6.73]} \\
 & Light Cells & 0.37 & \scriptsize\textcolor{gray!60}{[0.36,0.38]} & 0.37 & \scriptsize\textcolor{gray!60}{[0.36,0.39]} & 0.38 & \scriptsize\textcolor{gray!60}{[0.37,0.38]} & 0.34 & \scriptsize\textcolor{gray!60}{[0.31,0.37]} & 0.34 & \scriptsize\textcolor{gray!60}{[0.31,0.37]} & 0.34 & \scriptsize\textcolor{gray!60}{[0.30,0.37]} \\
 & Scroll & 0.25 & \scriptsize\textcolor{gray!60}{[0.24,0.27]} & 0.26 & \scriptsize\textcolor{gray!60}{[0.24,0.28]} & 0.26 & \scriptsize\textcolor{gray!60}{[0.25,0.28]} & 0.11 & \scriptsize\textcolor{gray!60}{[0.10,0.12]} & 0.11 & \scriptsize\textcolor{gray!60}{[0.10,0.13]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.10,0.13]} \\
 & Scroll Btm & 0.32 & \scriptsize\textcolor{gray!60}{[0.32,0.33]} & 0.33 & \scriptsize\textcolor{gray!60}{[0.32,0.33]} & 0.32 & \scriptsize\textcolor{gray!60}{[0.31,0.33]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.13,0.15]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.13,0.15]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.13,0.15]} \\
 & Scroll Btm
(small) & 0.32 & \scriptsize\textcolor{gray!60}{[0.31,0.33]} & 0.33 & \scriptsize\textcolor{gray!60}{[0.32,0.33]} & 0.32 & \scriptsize\textcolor{gray!60}{[0.31,0.34]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.13,0.16]} & 0.15 & \scriptsize\textcolor{gray!60}{[0.14,0.16]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.13,0.16]} \\
 & Scroll
(fullscreen) & 0.38 & \scriptsize\textcolor{gray!60}{[0.37,0.38]} & 0.39 & \scriptsize\textcolor{gray!60}{[0.38,0.40]} & 0.38 & \scriptsize\textcolor{gray!60}{[0.37,0.39]} & 0.24 & \scriptsize\textcolor{gray!60}{[0.22,0.26]} & 0.28 & \scriptsize\textcolor{gray!60}{[0.25,0.30]} & 0.22 & \scriptsize\textcolor{gray!60}{[0.20,0.25]} \\
 & Scroll Top & 0.25 & \scriptsize\textcolor{gray!60}{[0.23,0.26]} & 0.26 & \scriptsize\textcolor{gray!60}{[0.24,0.28]} & 0.24 & \scriptsize\textcolor{gray!60}{[0.22,0.26]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.10,0.13]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.10,0.14]} & 0.11 & \scriptsize\textcolor{gray!60}{[0.09,0.12]} \\
 & Scroll Top
(small) & 0.32 & \scriptsize\textcolor{gray!60}{[0.32,0.33]} & 0.32 & \scriptsize\textcolor{gray!60}{[0.32,0.33]} & 0.33 & \scriptsize\textcolor{gray!60}{[0.32,0.33]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.13,0.15]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.14,0.15]} & 0.15 & \scriptsize\textcolor{gray!60}{[0.14,0.16]} \\
 & Unicode & 0.23 & \scriptsize\textcolor{gray!60}{[0.21,0.24]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.26,0.28]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.25,0.28]} & 0.10 & \scriptsize\textcolor{gray!60}{[0.09,0.12]} & 0.13 & \scriptsize\textcolor{gray!60}{[0.11,0.14]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.11,0.13]} \\
\midrule
\multirow{7}{*}{\rotatebox{90}{fd}} & Cmd Exec. & 1.29 & \scriptsize\textcolor{gray!60}{[1.27,1.30]} & 1.28 & \scriptsize\textcolor{gray!60}{[1.27,1.30]} & 1.29 & \scriptsize\textcolor{gray!60}{[1.27,1.30]} & 1.05 & \scriptsize\textcolor{gray!60}{[1.04,1.07]} & 1.12 & \scriptsize\textcolor{gray!60}{[1.10,1.13]} & 1.12 & \scriptsize\textcolor{gray!60}{[1.11,1.14]} \\
 & Cmd Exec.
(large output) & 1.24 & \scriptsize\textcolor{gray!60}{[1.23,1.25]} & 1.25 & \scriptsize\textcolor{gray!60}{[1.22,1.28]} & 1.26 & \scriptsize\textcolor{gray!60}{[1.24,1.27]} & 1.02 & \scriptsize\textcolor{gray!60}{[1.01,1.04]} & 1.10 & \scriptsize\textcolor{gray!60}{[1.07,1.13]} & 1.11 & \scriptsize\textcolor{gray!60}{[1.10,1.13]} \\
 & File Extension & 0.13 & \scriptsize\textcolor{gray!60}{[0.13,0.13]} & 0.15 & \scriptsize\textcolor{gray!60}{[0.14,0.16]} & 0.13 & \scriptsize\textcolor{gray!60}{[0.13,0.14]} & 0.04 & \scriptsize\textcolor{gray!60}{[0.03,0.04]} & 0.04 & \scriptsize\textcolor{gray!60}{[0.04,0.05]} & 0.04 & \scriptsize\textcolor{gray!60}{[0.03,0.04]} \\
 & File Type & 0.12 & \scriptsize\textcolor{gray!60}{[0.12,0.13]} & 0.13 & \scriptsize\textcolor{gray!60}{[0.13,0.14]} & 0.13 & \scriptsize\textcolor{gray!60}{[0.12,0.13]} & 0.03 & \scriptsize\textcolor{gray!60}{[0.02,0.04]} & 0.04 & \scriptsize\textcolor{gray!60}{[0.03,0.04]} & 0.04 & \scriptsize\textcolor{gray!60}{[0.03,0.04]} \\
 & No Pattern & 0.18 & \scriptsize\textcolor{gray!60}{[0.18,0.19]} & 0.29 & \scriptsize\textcolor{gray!60}{[0.27,0.31]} & 0.22 & \scriptsize\textcolor{gray!60}{[0.21,0.23]} & 0.16 & \scriptsize\textcolor{gray!60}{[0.15,0.17]} & 0.29 & \scriptsize\textcolor{gray!60}{[0.27,0.30]} & 0.23 & \scriptsize\textcolor{gray!60}{[0.22,0.25]} \\
 & Simple & 0.27 & \scriptsize\textcolor{gray!60}{[0.26,0.27]} & 0.33 & \scriptsize\textcolor{gray!60}{[0.32,0.34]} & 0.32 & \scriptsize\textcolor{gray!60}{[0.31,0.32]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.13,0.15]} & 0.18 & \scriptsize\textcolor{gray!60}{[0.17,0.19]} & 0.16 & \scriptsize\textcolor{gray!60}{[0.15,0.17]} \\
 & Simple (-HI) & 0.12 & \scriptsize\textcolor{gray!60}{[0.12,0.13]} & 0.15 & \scriptsize\textcolor{gray!60}{[0.14,0.15]} & 0.13 & \scriptsize\textcolor{gray!60}{[0.13,0.13]} & 0.03 & \scriptsize\textcolor{gray!60}{[0.02,0.03]} & 0.04 & \scriptsize\textcolor{gray!60}{[0.03,0.04]} & 0.04 & \scriptsize\textcolor{gray!60}{[0.03,0.04]} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{grmtools}} & Eclipse & 3.48 & \scriptsize\textcolor{gray!60}{[3.46,3.51]} & 3.44 & \scriptsize\textcolor{gray!60}{[3.41,3.48]} & 3.74 & \scriptsize\textcolor{gray!60}{[3.70,3.78]} & 3.32 & \scriptsize\textcolor{gray!60}{[3.29,3.35]} & 3.28 & \scriptsize\textcolor{gray!60}{[3.24,3.31]} & 3.59 & \scriptsize\textcolor{gray!60}{[3.55,3.64]} \\
 & Hadoop & 2.86 & \scriptsize\textcolor{gray!60}{[2.85,2.87]} & 2.92 & \scriptsize\textcolor{gray!60}{[2.91,2.93]} & 3.09 & \scriptsize\textcolor{gray!60}{[3.08,3.10]} & 2.77 & \scriptsize\textcolor{gray!60}{[2.76,2.78]} & 2.80 & \scriptsize\textcolor{gray!60}{[2.79,2.81]} & 2.99 & \scriptsize\textcolor{gray!60}{[2.98,3.00]} \\
 & Jenkins & 2.90 & \scriptsize\textcolor{gray!60}{[2.90,2.91]} & 2.99 & \scriptsize\textcolor{gray!60}{[2.94,3.04]} & 3.02 & \scriptsize\textcolor{gray!60}{[3.01,3.03]} & 2.74 & \scriptsize\textcolor{gray!60}{[2.73,2.75]} & 2.81 & \scriptsize\textcolor{gray!60}{[2.77,2.84]} & 2.90 & \scriptsize\textcolor{gray!60}{[2.89,2.91]} \\
 & Spring & 2.43 & \scriptsize\textcolor{gray!60}{[2.42,2.43]} & 2.51 & \scriptsize\textcolor{gray!60}{[2.51,2.52]} & 2.63 & \scriptsize\textcolor{gray!60}{[2.61,2.65]} & 2.35 & \scriptsize\textcolor{gray!60}{[2.35,2.36]} & 2.40 & \scriptsize\textcolor{gray!60}{[2.39,2.41]} & 2.54 & \scriptsize\textcolor{gray!60}{[2.53,2.56]} \\
\midrule
\multirow{13}{*}{\rotatebox{90}{ripgrep}} & Alternates & 1.18 & \scriptsize\textcolor{gray!60}{[1.18,1.19]} & 1.29 & \scriptsize\textcolor{gray!60}{[1.28,1.31]} & 1.21 & \scriptsize\textcolor{gray!60}{[1.20,1.22]} & 0.42 & \scriptsize\textcolor{gray!60}{[0.40,0.44]} & 0.51 & \scriptsize\textcolor{gray!60}{[0.49,0.53]} & 0.43 & \scriptsize\textcolor{gray!60}{[0.41,0.44]} \\
 & Alternates
(no-case) & 1.31 & \scriptsize\textcolor{gray!60}{[1.30,1.31]} & 1.42 & \scriptsize\textcolor{gray!60}{[1.41,1.43]} & 1.33 & \scriptsize\textcolor{gray!60}{[1.33,1.34]} & 0.54 & \scriptsize\textcolor{gray!60}{[0.51,0.56]} & 0.65 & \scriptsize\textcolor{gray!60}{[0.63,0.67]} & 0.57 & \scriptsize\textcolor{gray!60}{[0.55,0.58]} \\
 & Literal & 1.12 & \scriptsize\textcolor{gray!60}{[1.11,1.12]} & 1.23 & \scriptsize\textcolor{gray!60}{[1.22,1.25]} & 1.15 & \scriptsize\textcolor{gray!60}{[1.14,1.15]} & 0.34 & \scriptsize\textcolor{gray!60}{[0.32,0.35]} & 0.44 & \scriptsize\textcolor{gray!60}{[0.43,0.46]} & 0.36 & \scriptsize\textcolor{gray!60}{[0.35,0.38]} \\
 & Literal
(no-case) & 1.19 & \scriptsize\textcolor{gray!60}{[1.19,1.19]} & 1.27 & \scriptsize\textcolor{gray!60}{[1.26,1.29]} & 1.20 & \scriptsize\textcolor{gray!60}{[1.20,1.21]} & 0.41 & \scriptsize\textcolor{gray!60}{[0.40,0.43]} & 0.50 & \scriptsize\textcolor{gray!60}{[0.48,0.52]} & 0.44 & \scriptsize\textcolor{gray!60}{[0.43,0.46]} \\
 & mmap
(no-case) & 1.67 & \scriptsize\textcolor{gray!60}{[1.66,1.68]} & 1.80 & \scriptsize\textcolor{gray!60}{[1.78,1.81]} & 1.72 & \scriptsize\textcolor{gray!60}{[1.71,1.72]} & 0.48 & \scriptsize\textcolor{gray!60}{[0.46,0.49]} & 0.58 & \scriptsize\textcolor{gray!60}{[0.56,0.60]} & 0.50 & \scriptsize\textcolor{gray!60}{[0.48,0.52]} \\
 & Literal
(default) & 1.08 & \scriptsize\textcolor{gray!60}{[1.07,1.09]} & 1.19 & \scriptsize\textcolor{gray!60}{[1.18,1.20]} & 1.10 & \scriptsize\textcolor{gray!60}{[1.10,1.11]} & 0.30 & \scriptsize\textcolor{gray!60}{[0.29,0.32]} & 0.40 & \scriptsize\textcolor{gray!60}{[0.39,0.41]} & 0.32 & \scriptsize\textcolor{gray!60}{[0.31,0.33]} \\
 & mmap & 1.64 & \scriptsize\textcolor{gray!60}{[1.63,1.64]} & 1.75 & \scriptsize\textcolor{gray!60}{[1.74,1.77]} & 1.67 & \scriptsize\textcolor{gray!60}{[1.67,1.68]} & 0.43 & \scriptsize\textcolor{gray!60}{[0.41,0.45]} & 0.52 & \scriptsize\textcolor{gray!60}{[0.50,0.54]} & 0.46 & \scriptsize\textcolor{gray!60}{[0.44,0.47]} \\
 & Literal
(Regex) & 1.13 & \scriptsize\textcolor{gray!60}{[1.12,1.14]} & 1.25 & \scriptsize\textcolor{gray!60}{[1.24,1.26]} & 1.15 & \scriptsize\textcolor{gray!60}{[1.15,1.16]} & 0.35 & \scriptsize\textcolor{gray!60}{[0.33,0.36]} & 0.44 & \scriptsize\textcolor{gray!60}{[0.43,0.46]} & 0.36 & \scriptsize\textcolor{gray!60}{[0.35,0.38]} \\
 & UTF Greek & 3.29 & \scriptsize\textcolor{gray!60}{[3.28,3.30]} & 3.41 & \scriptsize\textcolor{gray!60}{[3.39,3.42]} & 3.33 & \scriptsize\textcolor{gray!60}{[3.32,3.33]} & 2.55 & \scriptsize\textcolor{gray!60}{[2.53,2.57]} & 2.64 & \scriptsize\textcolor{gray!60}{[2.62,2.66]} & 2.58 & \scriptsize\textcolor{gray!60}{[2.55,2.61]} \\
 & UTF Greek
(no-case) & 3.30 & \scriptsize\textcolor{gray!60}{[3.29,3.31]} & 3.42 & \scriptsize\textcolor{gray!60}{[3.39,3.44]} & 3.33 & \scriptsize\textcolor{gray!60}{[3.32,3.34]} & 2.56 & \scriptsize\textcolor{gray!60}{[2.53,2.59]} & 2.66 & \scriptsize\textcolor{gray!60}{[2.63,2.69]} & 2.56 & \scriptsize\textcolor{gray!60}{[2.53,2.58]} \\
 & UTF Word & 1.09 & \scriptsize\textcolor{gray!60}{[1.08,1.10]} & 1.21 & \scriptsize\textcolor{gray!60}{[1.20,1.22]} & 1.14 & \scriptsize\textcolor{gray!60}{[1.13,1.14]} & 0.35 & \scriptsize\textcolor{gray!60}{[0.33,0.37]} & 0.42 & \scriptsize\textcolor{gray!60}{[0.40,0.43]} & 0.37 & \scriptsize\textcolor{gray!60}{[0.36,0.39]} \\
 & UTF Word
(alt.) & 1.11 & \scriptsize\textcolor{gray!60}{[1.10,1.11]} & 1.21 & \scriptsize\textcolor{gray!60}{[1.20,1.22]} & 1.13 & \scriptsize\textcolor{gray!60}{[1.13,1.14]} & 0.33 & \scriptsize\textcolor{gray!60}{[0.32,0.35]} & 0.43 & \scriptsize\textcolor{gray!60}{[0.41,0.45]} & 0.35 & \scriptsize\textcolor{gray!60}{[0.33,0.36]} \\
 & Word & 1.12 & \scriptsize\textcolor{gray!60}{[1.11,1.12]} & 1.22 & \scriptsize\textcolor{gray!60}{[1.21,1.24]} & 1.14 & \scriptsize\textcolor{gray!60}{[1.13,1.14]} & 0.35 & \scriptsize\textcolor{gray!60}{[0.34,0.37]} & 0.43 & \scriptsize\textcolor{gray!60}{[0.42,0.45]} & 0.36 & \scriptsize\textcolor{gray!60}{[0.35,0.37]} \\
\midrule
\multirow{26}{*}{\rotatebox{90}{som-rs-ast}} & Bounce & 0.62 & \scriptsize\textcolor{gray!60}{[0.62,0.62]} & 0.96 & \scriptsize\textcolor{gray!60}{[0.94,0.98]} & 0.80 & \scriptsize\textcolor{gray!60}{[0.79,0.80]} & 0.62 & \scriptsize\textcolor{gray!60}{[0.61,0.62]} & 0.96 & \scriptsize\textcolor{gray!60}{[0.94,0.97]} & 0.79 & \scriptsize\textcolor{gray!60}{[0.79,0.79]} \\
 & BubbleSort & 0.56 & \scriptsize\textcolor{gray!60}{[0.56,0.57]} & 0.84 & \scriptsize\textcolor{gray!60}{[0.83,0.85]} & 0.71 & \scriptsize\textcolor{gray!60}{[0.71,0.72]} & 0.56 & \scriptsize\textcolor{gray!60}{[0.55,0.56]} & 0.83 & \scriptsize\textcolor{gray!60}{[0.82,0.84]} & 0.71 & \scriptsize\textcolor{gray!60}{[0.71,0.71]} \\
 & DeltaBlue & 0.77 & \scriptsize\textcolor{gray!60}{[0.77,0.78]} & 1.09 & \scriptsize\textcolor{gray!60}{[1.08,1.10]} & 0.98 & \scriptsize\textcolor{gray!60}{[0.98,0.98]} & 0.77 & \scriptsize\textcolor{gray!60}{[0.76,0.77]} & 1.07 & \scriptsize\textcolor{gray!60}{[1.06,1.08]} & 0.97 & \scriptsize\textcolor{gray!60}{[0.97,0.98]} \\
 & Dispatch & 0.59 & \scriptsize\textcolor{gray!60}{[0.58,0.60]} & 0.97 & \scriptsize\textcolor{gray!60}{[0.97,0.97]} & 0.77 & \scriptsize\textcolor{gray!60}{[0.76,0.77]} & 0.59 & \scriptsize\textcolor{gray!60}{[0.58,0.59]} & 0.96 & \scriptsize\textcolor{gray!60}{[0.96,0.97]} & 0.76 & \scriptsize\textcolor{gray!60}{[0.75,0.77]} \\
 & Fannkuch & 0.65 & \scriptsize\textcolor{gray!60}{[0.64,0.65]} & 1.01 & \scriptsize\textcolor{gray!60}{[0.95,1.07]} & 0.81 & \scriptsize\textcolor{gray!60}{[0.80,0.81]} & 0.64 & \scriptsize\textcolor{gray!60}{[0.64,0.65]} & 0.98 & \scriptsize\textcolor{gray!60}{[0.93,1.04]} & 0.80 & \scriptsize\textcolor{gray!60}{[0.80,0.81]} \\
 & Fibonacci & 0.83 & \scriptsize\textcolor{gray!60}{[0.82,0.83]} & 1.41 & \scriptsize\textcolor{gray!60}{[1.40,1.41]} & 1.08 & \scriptsize\textcolor{gray!60}{[1.07,1.08]} & 0.82 & \scriptsize\textcolor{gray!60}{[0.82,0.83]} & 1.40 & \scriptsize\textcolor{gray!60}{[1.40,1.41]} & 1.07 & \scriptsize\textcolor{gray!60}{[1.07,1.08]} \\
 & FieldLoop & 0.94 & \scriptsize\textcolor{gray!60}{[0.94,0.95]} & 1.20 & \scriptsize\textcolor{gray!60}{[1.20,1.21]} & 1.07 & \scriptsize\textcolor{gray!60}{[1.07,1.08]} & 0.94 & \scriptsize\textcolor{gray!60}{[0.93,0.94]} & 1.20 & \scriptsize\textcolor{gray!60}{[1.19,1.21]} & 1.07 & \scriptsize\textcolor{gray!60}{[1.06,1.07]} \\
 & GraphSearch & 0.31 & \scriptsize\textcolor{gray!60}{[0.30,0.31]} & 0.43 & \scriptsize\textcolor{gray!60}{[0.43,0.44]} & 0.38 & \scriptsize\textcolor{gray!60}{[0.38,0.39]} & 0.30 & \scriptsize\textcolor{gray!60}{[0.29,0.30]} & 0.41 & \scriptsize\textcolor{gray!60}{[0.40,0.42]} & 0.37 & \scriptsize\textcolor{gray!60}{[0.37,0.38]} \\
 & IntegerLoop & 0.52 & \scriptsize\textcolor{gray!60}{[0.51,0.53]} & 0.84 & \scriptsize\textcolor{gray!60}{[0.84,0.84]} & 0.67 & \scriptsize\textcolor{gray!60}{[0.66,0.67]} & 0.52 & \scriptsize\textcolor{gray!60}{[0.51,0.52]} & 0.83 & \scriptsize\textcolor{gray!60}{[0.83,0.84]} & 0.66 & \scriptsize\textcolor{gray!60}{[0.66,0.67]} \\
 & JsonSmall & 0.86 & \scriptsize\textcolor{gray!60}{[0.85,0.86]} & 1.22 & \scriptsize\textcolor{gray!60}{[1.22,1.23]} & 1.10 & \scriptsize\textcolor{gray!60}{[1.10,1.11]} & 0.85 & \scriptsize\textcolor{gray!60}{[0.84,0.85]} & 1.21 & \scriptsize\textcolor{gray!60}{[1.20,1.21]} & 1.10 & \scriptsize\textcolor{gray!60}{[1.09,1.10]} \\
 & List & 0.38 & \scriptsize\textcolor{gray!60}{[0.38,0.39]} & 0.53 & \scriptsize\textcolor{gray!60}{[0.52,0.54]} & 0.48 & \scriptsize\textcolor{gray!60}{[0.47,0.48]} & 0.38 & \scriptsize\textcolor{gray!60}{[0.37,0.38]} & 0.52 & \scriptsize\textcolor{gray!60}{[0.52,0.53]} & 0.47 & \scriptsize\textcolor{gray!60}{[0.47,0.48]} \\
 & Loop & 0.53 & \scriptsize\textcolor{gray!60}{[0.52,0.53]} & 0.86 & \scriptsize\textcolor{gray!60}{[0.84,0.87]} & 0.70 & \scriptsize\textcolor{gray!60}{[0.70,0.71]} & 0.52 & \scriptsize\textcolor{gray!60}{[0.52,0.53]} & 0.85 & \scriptsize\textcolor{gray!60}{[0.84,0.86]} & 0.70 & \scriptsize\textcolor{gray!60}{[0.70,0.70]} \\
 & Mandelbrot & 0.46 & \scriptsize\textcolor{gray!60}{[0.45,0.46]} & 0.69 & \scriptsize\textcolor{gray!60}{[0.68,0.70]} & 0.57 & \scriptsize\textcolor{gray!60}{[0.57,0.57]} & 0.45 & \scriptsize\textcolor{gray!60}{[0.45,0.46]} & 0.69 & \scriptsize\textcolor{gray!60}{[0.68,0.70]} & 0.57 & \scriptsize\textcolor{gray!60}{[0.56,0.57]} \\
 & NBody & 0.31 & \scriptsize\textcolor{gray!60}{[0.31,0.31]} & 0.38 & \scriptsize\textcolor{gray!60}{[0.38,0.39]} & 0.34 & \scriptsize\textcolor{gray!60}{[0.34,0.34]} & 0.31 & \scriptsize\textcolor{gray!60}{[0.30,0.31]} & 0.38 & \scriptsize\textcolor{gray!60}{[0.37,0.38]} & 0.34 & \scriptsize\textcolor{gray!60}{[0.33,0.34]} \\
 & PageRank & 0.31 & \scriptsize\textcolor{gray!60}{[0.31,0.31]} & 0.44 & \scriptsize\textcolor{gray!60}{[0.43,0.44]} & 0.39 & \scriptsize\textcolor{gray!60}{[0.38,0.39]} & 0.30 & \scriptsize\textcolor{gray!60}{[0.30,0.30]} & 0.43 & \scriptsize\textcolor{gray!60}{[0.43,0.44]} & 0.38 & \scriptsize\textcolor{gray!60}{[0.38,0.39]} \\
 & Permute & 0.67 & \scriptsize\textcolor{gray!60}{[0.66,0.67]} & 0.90 & \scriptsize\textcolor{gray!60}{[0.88,0.91]} & 0.82 & \scriptsize\textcolor{gray!60}{[0.82,0.82]} & 0.66 & \scriptsize\textcolor{gray!60}{[0.66,0.66]} & 0.89 & \scriptsize\textcolor{gray!60}{[0.87,0.91]} & 0.82 & \scriptsize\textcolor{gray!60}{[0.81,0.82]} \\
 & Queens & 0.77 & \scriptsize\textcolor{gray!60}{[0.77,0.78]} & 1.18 & \scriptsize\textcolor{gray!60}{[1.16,1.21]} & 0.98 & \scriptsize\textcolor{gray!60}{[0.97,0.98]} & 0.77 & \scriptsize\textcolor{gray!60}{[0.76,0.77]} & 1.18 & \scriptsize\textcolor{gray!60}{[1.16,1.20]} & 0.97 & \scriptsize\textcolor{gray!60}{[0.97,0.98]} \\
 & QuickSort & 0.98 & \scriptsize\textcolor{gray!60}{[0.98,0.98]} & 1.27 & \scriptsize\textcolor{gray!60}{[1.26,1.29]} & 1.26 & \scriptsize\textcolor{gray!60}{[1.26,1.27]} & 0.98 & \scriptsize\textcolor{gray!60}{[0.97,0.98]} & 1.26 & \scriptsize\textcolor{gray!60}{[1.25,1.28]} & 1.26 & \scriptsize\textcolor{gray!60}{[1.26,1.27]} \\
 & Recurse & 0.60 & \scriptsize\textcolor{gray!60}{[0.59,0.60]} & 0.92 & \scriptsize\textcolor{gray!60}{[0.92,0.92]} & 0.79 & \scriptsize\textcolor{gray!60}{[0.79,0.80]} & 0.60 & \scriptsize\textcolor{gray!60}{[0.59,0.60]} & 0.91 & \scriptsize\textcolor{gray!60}{[0.91,0.92]} & 0.79 & \scriptsize\textcolor{gray!60}{[0.79,0.79]} \\
 & Richards & 2.48 & \scriptsize\textcolor{gray!60}{[2.46,2.49]} & 3.72 & \scriptsize\textcolor{gray!60}{[3.61,3.83]} & 3.13 & \scriptsize\textcolor{gray!60}{[3.12,3.14]} & 2.47 & \scriptsize\textcolor{gray!60}{[2.46,2.49]} & 3.72 & \scriptsize\textcolor{gray!60}{[3.61,3.82]} & 3.13 & \scriptsize\textcolor{gray!60}{[3.12,3.14]} \\
 & Sieve & 0.67 & \scriptsize\textcolor{gray!60}{[0.66,0.67]} & 0.94 & \scriptsize\textcolor{gray!60}{[0.94,0.95]} & 0.87 & \scriptsize\textcolor{gray!60}{[0.87,0.88]} & 0.66 & \scriptsize\textcolor{gray!60}{[0.66,0.67]} & 0.94 & \scriptsize\textcolor{gray!60}{[0.93,0.94]} & 0.87 & \scriptsize\textcolor{gray!60}{[0.86,0.87]} \\
 & Storage & 0.56 & \scriptsize\textcolor{gray!60}{[0.55,0.56]} & 0.70 & \scriptsize\textcolor{gray!60}{[0.69,0.71]} & 0.69 & \scriptsize\textcolor{gray!60}{[0.69,0.69]} & 0.55 & \scriptsize\textcolor{gray!60}{[0.55,0.56]} & 0.69 & \scriptsize\textcolor{gray!60}{[0.68,0.69]} & 0.68 & \scriptsize\textcolor{gray!60}{[0.68,0.69]} \\
 & Sum & 0.52 & \scriptsize\textcolor{gray!60}{[0.52,0.53]} & 0.83 & \scriptsize\textcolor{gray!60}{[0.81,0.84]} & 0.67 & \scriptsize\textcolor{gray!60}{[0.67,0.68]} & 0.52 & \scriptsize\textcolor{gray!60}{[0.51,0.52]} & 0.82 & \scriptsize\textcolor{gray!60}{[0.81,0.83]} & 0.67 & \scriptsize\textcolor{gray!60}{[0.66,0.67]} \\
 & Towers & 0.31 & \scriptsize\textcolor{gray!60}{[0.31,0.31]} & 0.46 & \scriptsize\textcolor{gray!60}{[0.45,0.47]} & 0.38 & \scriptsize\textcolor{gray!60}{[0.38,0.39]} & 0.31 & \scriptsize\textcolor{gray!60}{[0.30,0.31]} & 0.46 & \scriptsize\textcolor{gray!60}{[0.45,0.46]} & 0.38 & \scriptsize\textcolor{gray!60}{[0.37,0.38]} \\
 & TreeSort & 0.32 & \scriptsize\textcolor{gray!60}{[0.31,0.32]} & 0.41 & \scriptsize\textcolor{gray!60}{[0.41,0.42]} & 0.40 & \scriptsize\textcolor{gray!60}{[0.40,0.40]} & 0.31 & \scriptsize\textcolor{gray!60}{[0.31,0.32]} & 0.40 & \scriptsize\textcolor{gray!60}{[0.39,0.40]} & 0.40 & \scriptsize\textcolor{gray!60}{[0.39,0.40]} \\
 & WhileLoop & 0.48 & \scriptsize\textcolor{gray!60}{[0.47,0.48]} & 0.72 & \scriptsize\textcolor{gray!60}{[0.72,0.73]} & 0.60 & \scriptsize\textcolor{gray!60}{[0.59,0.60]} & 0.47 & \scriptsize\textcolor{gray!60}{[0.47,0.48]} & 0.72 & \scriptsize\textcolor{gray!60}{[0.72,0.72]} & 0.59 & \scriptsize\textcolor{gray!60}{[0.59,0.60]} \\
\midrule
\multirow{26}{*}{\rotatebox{90}{som-rs-bc}} & Bounce & 0.25 & \scriptsize\textcolor{gray!60}{[0.24,0.25]} & 0.28 & \scriptsize\textcolor{gray!60}{[0.28,0.29]} & 0.30 & \scriptsize\textcolor{gray!60}{[0.29,0.30]} & 0.25 & \scriptsize\textcolor{gray!60}{[0.24,0.25]} & 0.28 & \scriptsize\textcolor{gray!60}{[0.28,0.28]} & 0.29 & \scriptsize\textcolor{gray!60}{[0.29,0.30]} \\
 & BubbleSort & 0.23 & \scriptsize\textcolor{gray!60}{[0.23,0.23]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.27,0.28]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.26,0.27]} & 0.22 & \scriptsize\textcolor{gray!60}{[0.22,0.22]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.27,0.27]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.26,0.27]} \\
 & DeltaBlue & 0.30 & \scriptsize\textcolor{gray!60}{[0.29,0.30]} & 0.34 & \scriptsize\textcolor{gray!60}{[0.34,0.35]} & 0.36 & \scriptsize\textcolor{gray!60}{[0.35,0.36]} & 0.30 & \scriptsize\textcolor{gray!60}{[0.29,0.30]} & 0.34 & \scriptsize\textcolor{gray!60}{[0.33,0.34]} & 0.35 & \scriptsize\textcolor{gray!60}{[0.35,0.36]} \\
 & Dispatch & 0.25 & \scriptsize\textcolor{gray!60}{[0.25,0.25]} & 0.28 & \scriptsize\textcolor{gray!60}{[0.28,0.29]} & 0.29 & \scriptsize\textcolor{gray!60}{[0.29,0.30]} & 0.24 & \scriptsize\textcolor{gray!60}{[0.24,0.25]} & 0.28 & \scriptsize\textcolor{gray!60}{[0.28,0.28]} & 0.29 & \scriptsize\textcolor{gray!60}{[0.29,0.30]} \\
 & Fannkuch & 0.25 & \scriptsize\textcolor{gray!60}{[0.24,0.25]} & 0.29 & \scriptsize\textcolor{gray!60}{[0.29,0.29]} & 0.29 & \scriptsize\textcolor{gray!60}{[0.28,0.29]} & 0.24 & \scriptsize\textcolor{gray!60}{[0.24,0.25]} & 0.28 & \scriptsize\textcolor{gray!60}{[0.28,0.29]} & 0.28 & \scriptsize\textcolor{gray!60}{[0.28,0.28]} \\
 & Fibonacci & 0.30 & \scriptsize\textcolor{gray!60}{[0.30,0.31]} & 0.37 & \scriptsize\textcolor{gray!60}{[0.36,0.37]} & 0.36 & \scriptsize\textcolor{gray!60}{[0.36,0.37]} & 0.30 & \scriptsize\textcolor{gray!60}{[0.29,0.30]} & 0.36 & \scriptsize\textcolor{gray!60}{[0.36,0.37]} & 0.36 & \scriptsize\textcolor{gray!60}{[0.35,0.36]} \\
 & FieldLoop & 0.49 & \scriptsize\textcolor{gray!60}{[0.48,0.49]} & 0.43 & \scriptsize\textcolor{gray!60}{[0.42,0.43]} & 0.54 & \scriptsize\textcolor{gray!60}{[0.53,0.55]} & 0.48 & \scriptsize\textcolor{gray!60}{[0.48,0.49]} & 0.42 & \scriptsize\textcolor{gray!60}{[0.42,0.43]} & 0.53 & \scriptsize\textcolor{gray!60}{[0.52,0.54]} \\
 & GraphSearch & 0.12 & \scriptsize\textcolor{gray!60}{[0.12,0.12]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.12,0.13]} & 0.15 & \scriptsize\textcolor{gray!60}{[0.14,0.15]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.11,0.12]} & 0.11 & \scriptsize\textcolor{gray!60}{[0.11,0.11]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.13,0.14]} \\
 & IntegerLoop & 0.22 & \scriptsize\textcolor{gray!60}{[0.22,0.22]} & 0.24 & \scriptsize\textcolor{gray!60}{[0.24,0.25]} & 0.26 & \scriptsize\textcolor{gray!60}{[0.26,0.26]} & 0.22 & \scriptsize\textcolor{gray!60}{[0.21,0.22]} & 0.24 & \scriptsize\textcolor{gray!60}{[0.24,0.24]} & 0.26 & \scriptsize\textcolor{gray!60}{[0.26,0.26]} \\
 & JsonSmall & 0.37 & \scriptsize\textcolor{gray!60}{[0.36,0.37]} & 0.39 & \scriptsize\textcolor{gray!60}{[0.39,0.40]} & 0.44 & \scriptsize\textcolor{gray!60}{[0.44,0.44]} & 0.36 & \scriptsize\textcolor{gray!60}{[0.36,0.37]} & 0.39 & \scriptsize\textcolor{gray!60}{[0.38,0.39]} & 0.44 & \scriptsize\textcolor{gray!60}{[0.43,0.44]} \\
 & List & 0.18 & \scriptsize\textcolor{gray!60}{[0.17,0.18]} & 0.22 & \scriptsize\textcolor{gray!60}{[0.22,0.23]} & 0.21 & \scriptsize\textcolor{gray!60}{[0.20,0.21]} & 0.17 & \scriptsize\textcolor{gray!60}{[0.17,0.18]} & 0.22 & \scriptsize\textcolor{gray!60}{[0.22,0.22]} & 0.21 & \scriptsize\textcolor{gray!60}{[0.20,0.21]} \\
 & Loop & 0.23 & \scriptsize\textcolor{gray!60}{[0.22,0.23]} & 0.26 & \scriptsize\textcolor{gray!60}{[0.25,0.26]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.26,0.27]} & 0.22 & \scriptsize\textcolor{gray!60}{[0.21,0.22]} & 0.25 & \scriptsize\textcolor{gray!60}{[0.24,0.25]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.26,0.27]} \\
 & Mandelbrot & 0.20 & \scriptsize\textcolor{gray!60}{[0.19,0.20]} & 0.22 & \scriptsize\textcolor{gray!60}{[0.21,0.22]} & 0.23 & \scriptsize\textcolor{gray!60}{[0.23,0.24]} & 0.19 & \scriptsize\textcolor{gray!60}{[0.19,0.19]} & 0.21 & \scriptsize\textcolor{gray!60}{[0.20,0.22]} & 0.23 & \scriptsize\textcolor{gray!60}{[0.23,0.23]} \\
 & NBody & 0.11 & \scriptsize\textcolor{gray!60}{[0.11,0.12]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.12,0.12]} & 0.13 & \scriptsize\textcolor{gray!60}{[0.12,0.13]} & 0.11 & \scriptsize\textcolor{gray!60}{[0.11,0.11]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.11,0.12]} & 0.13 & \scriptsize\textcolor{gray!60}{[0.12,0.13]} \\
 & PageRank & 0.13 & \scriptsize\textcolor{gray!60}{[0.12,0.13]} & 0.13 & \scriptsize\textcolor{gray!60}{[0.13,0.13]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.14,0.15]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.12,0.12]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.12,0.13]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.13,0.14]} \\
 & Permute & 0.24 & \scriptsize\textcolor{gray!60}{[0.23,0.24]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.27,0.27]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.27,0.27]} & 0.23 & \scriptsize\textcolor{gray!60}{[0.23,0.24]} & 0.26 & \scriptsize\textcolor{gray!60}{[0.26,0.27]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.27,0.27]} \\
 & Queens & 0.28 & \scriptsize\textcolor{gray!60}{[0.27,0.28]} & 0.33 & \scriptsize\textcolor{gray!60}{[0.33,0.33]} & 0.33 & \scriptsize\textcolor{gray!60}{[0.33,0.33]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.27,0.28]} & 0.33 & \scriptsize\textcolor{gray!60}{[0.32,0.33]} & 0.33 & \scriptsize\textcolor{gray!60}{[0.32,0.33]} \\
 & QuickSort & 0.36 & \scriptsize\textcolor{gray!60}{[0.35,0.36]} & 0.38 & \scriptsize\textcolor{gray!60}{[0.38,0.38]} & 0.43 & \scriptsize\textcolor{gray!60}{[0.43,0.43]} & 0.35 & \scriptsize\textcolor{gray!60}{[0.35,0.36]} & 0.38 & \scriptsize\textcolor{gray!60}{[0.37,0.38]} & 0.42 & \scriptsize\textcolor{gray!60}{[0.42,0.43]} \\
 & Recurse & 0.25 & \scriptsize\textcolor{gray!60}{[0.25,0.26]} & 0.31 & \scriptsize\textcolor{gray!60}{[0.31,0.31]} & 0.30 & \scriptsize\textcolor{gray!60}{[0.30,0.31]} & 0.25 & \scriptsize\textcolor{gray!60}{[0.24,0.25]} & 0.31 & \scriptsize\textcolor{gray!60}{[0.30,0.31]} & 0.30 & \scriptsize\textcolor{gray!60}{[0.30,0.31]} \\
 & Richards & 0.92 & \scriptsize\textcolor{gray!60}{[0.92,0.93]} & 1.20 & \scriptsize\textcolor{gray!60}{[1.20,1.21]} & 1.10 & \scriptsize\textcolor{gray!60}{[1.10,1.11]} & 0.92 & \scriptsize\textcolor{gray!60}{[0.91,0.92]} & 1.20 & \scriptsize\textcolor{gray!60}{[1.19,1.20]} & 1.10 & \scriptsize\textcolor{gray!60}{[1.09,1.11]} \\
 & Sieve & 0.25 & \scriptsize\textcolor{gray!60}{[0.25,0.26]} & 0.26 & \scriptsize\textcolor{gray!60}{[0.26,0.27]} & 0.30 & \scriptsize\textcolor{gray!60}{[0.29,0.31]} & 0.25 & \scriptsize\textcolor{gray!60}{[0.24,0.25]} & 0.26 & \scriptsize\textcolor{gray!60}{[0.25,0.26]} & 0.30 & \scriptsize\textcolor{gray!60}{[0.29,0.31]} \\
 & Storage & 0.22 & \scriptsize\textcolor{gray!60}{[0.22,0.22]} & 0.21 & \scriptsize\textcolor{gray!60}{[0.20,0.21]} & 0.25 & \scriptsize\textcolor{gray!60}{[0.25,0.26]} & 0.22 & \scriptsize\textcolor{gray!60}{[0.21,0.22]} & 0.20 & \scriptsize\textcolor{gray!60}{[0.20,0.21]} & 0.25 & \scriptsize\textcolor{gray!60}{[0.25,0.25]} \\
 & Sum & 0.22 & \scriptsize\textcolor{gray!60}{[0.22,0.22]} & 0.25 & \scriptsize\textcolor{gray!60}{[0.25,0.25]} & 0.27 & \scriptsize\textcolor{gray!60}{[0.26,0.27]} & 0.22 & \scriptsize\textcolor{gray!60}{[0.22,0.22]} & 0.24 & \scriptsize\textcolor{gray!60}{[0.24,0.25]} & 0.26 & \scriptsize\textcolor{gray!60}{[0.26,0.27]} \\
 & Towers & 0.13 & \scriptsize\textcolor{gray!60}{[0.12,0.13]} & 0.15 & \scriptsize\textcolor{gray!60}{[0.14,0.15]} & 0.15 & \scriptsize\textcolor{gray!60}{[0.15,0.15]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.12,0.12]} & 0.15 & \scriptsize\textcolor{gray!60}{[0.14,0.15]} & 0.14 & \scriptsize\textcolor{gray!60}{[0.14,0.15]} \\
 & TreeSort & 0.11 & \scriptsize\textcolor{gray!60}{[0.10,0.11]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.11,0.12]} & 0.13 & \scriptsize\textcolor{gray!60}{[0.13,0.13]} & 0.11 & \scriptsize\textcolor{gray!60}{[0.10,0.11]} & 0.11 & \scriptsize\textcolor{gray!60}{[0.11,0.12]} & 0.12 & \scriptsize\textcolor{gray!60}{[0.12,0.12]} \\
 & WhileLoop & 0.22 & \scriptsize\textcolor{gray!60}{[0.22,0.22]} & 0.23 & \scriptsize\textcolor{gray!60}{[0.22,0.23]} & 0.25 & \scriptsize\textcolor{gray!60}{[0.25,0.26]} & 0.21 & \scriptsize\textcolor{gray!60}{[0.21,0.22]} & 0.22 & \scriptsize\textcolor{gray!60}{[0.22,0.23]} & 0.25 & \scriptsize\textcolor{gray!60}{[0.24,0.25]} \\
\bottomrule
\end{tabular}

==> tables/gcvs_user.tex <==
\begin{tabular}{l r@{\hspace{3pt}}l}
\toprule
Suite & \multicolumn{2}{c}{User time} \\
\midrule
alacritty & 0.263 & \scriptsize\textcolor{gray!60}{$\pm$0.064} \\
binary_trees & 0.082 & \scriptsize\textcolor{gray!60}{$\pm$0.003} \\
fd & 0.122 & \scriptsize\textcolor{gray!60}{$\pm$0.034} \\
grmtools & 2.773 & \scriptsize\textcolor{gray!60}{$\pm$0.063} \\
regex_redux & 0.502 & \scriptsize\textcolor{gray!60}{$\pm$0.006} \\
ripgrep & 0.515 & \scriptsize\textcolor{gray!60}{$\pm$0.040} \\
som-rs-ast & 0.570 & \scriptsize\textcolor{gray!60}{$\pm$0.031} \\
som-rs-bc & 0.229 & \scriptsize\textcolor{gray!60}{$\pm$0.008} \\
\bottomrule
\end{tabular}


==> tables/mem_dist_pct.tex <==
\begin{tabular}{lrrrr}
  \toprule
  & \multicolumn{3}{c}{Heap Distribution (\%)} & GC Transitive \\
  \cmidrule(lr){2-4}                      % ← thin rule under cols 2–4
        & \rc & \texttt{Box<T>} & \gc & \\ % second header row
  \midrule
  \alacritty   & 1.41 & 98.57 & 0.02 &  2.70 \\
  \binarytrees & 0.00 & 50.00 & 50.00 & 100.00 \\
  \fd          & 5.49 & 94.49 & 0.02 &  1.23 \\
  \grmtools    & 0.01 & 83.09 & 16.90 & 44.19 \\
  \regexredux  & 1.38 & 96.22 & 2.40 & 15.39 \\
  \ripgrep     & 2.28 & 93.06 & 4.65 & 17.97 \\
  \somrsast    & 0.00 & 84.85 & 15.15 & 76.95 \\
  \somrsbc     & 0.00 & 61.04 & 38.96 & 99.71 \\
  \bottomrule
\end{tabular}


